Deep Leakage from Gradients

Exchanging gradients is a widely used method in modern multi-node machine learning system (e.g., distributed training, collaborative learning). For a long time, people believed that gradients are safe to share: i.e., the training data will not be leaked by gradient exchange. However, we show that it is possible to obtain the private training data from the publicly shared gradients. We name this leakage as Deep Leakage from Gradient and empirically validate the effectiveness on both computer vision and natural language processing tasks. Experimental results show that our attack is much stronger than previous approaches: the recovery is pixel-wise accurate for images and token-wise matching for texts. We want to raise people's awareness to rethink the gradient's safety. Finally, we discuss several possible strategies to prevent such deep leakage. The most effective defense method is gradient pruning.

==> contents/proof.tex <==
\ligeng{TODO: format the notions.} \ligeng{Justify layer types.}

Let $X_\ell$ and $y_\ell$ be the input and output for $\ell^{th}$ layer. Given the weights $w_\ell$, the calculating process of inputs $X$ labels $Y$ can written as 

\begin{align*} 
    y_\ell &= f_\ell(X_\ell; w_\ell) \\
    % y_{\ell+1} &= f_{\ell + 1}(X_{\ell + 1}; w_{\ell + 1}) \\
    y &=   f_{N} ( f_{N-1} ( ... f_1 (X, w_1) ...w_{N-1} ) w_N) \\
      &= F(X, W)
\end{align*}

We care about the uniqueness between inputs $X, Y$ and gradients $\Delta W$. Is it possible that there is another pair of $X', Y'$ that produces the gradients that is same as previous?


\begin{equation}
    \frac{\partial Loss(F(X, W), Y)}{\partial W} = \frac{\partial Loss(F(X', W), Y')}{\partial W'} 
\end{equation}


Assume $j^{th}$ layer is a linear operation, for weight $w_j$

% $$
%     \frac{\partial Loss}{\partial w_{j}} = 
%     \frac{\partial Loss'}{\partial w_{j}}
% $$

\begin{equation}\label{eq:dldw_{j}}
    \frac{\partial Loss}{\partial y_{j}}
    \frac{\partial y_{j}}{\partial w_{j}}
    = 
    \frac{\partial Loss'}{\partial y'_{j}}
    \frac{\partial y'_{j}}{\partial w_{j}}
\end{equation}

For weight $w_{j-1}$

\begin{equation}\label{eq:dldw_{j-1}}
    \frac{\partial Loss}{\partial y_{j}}
    \frac{\partial y_{j}}{\partial y_{j-1}}
    \frac{\partial y_{j-1}}{\partial w_{j-1}}
    = 
    \frac{\partial Loss'}{\partial y'_{j}}
    \frac{\partial y'_{j}}{\partial y'_{j-1}}
    \frac{\partial y'_{j-1}}{\partial w'_{j-1}}
\end{equation}

Note, as $f_j()$ is a linear operation, $ \frac{\partial y_{j}}{\partial y_{j-1}}$ actually only relates with  $w_{j-1}$, regardless the inputs $ y_{j-1} $. The formula Eq.~\ref{eq:dldw_{j-1}} can be further simplified to 
 
\begin{equation}
    \frac{\partial Loss}{\partial y_{j}}
    % \frac{\partial y_{j}}{\partial y_{j-1}}
    \frac{\partial y_{j-1}}{\partial w_{j-1}}
    = 
    \frac{\partial Loss'}{\partial y'_{j}}
    % \frac{\partial y'_{j}}{\partial y'_{j-1}}
    \frac{\partial y'_{j-1}}{\partial w'_{j-1}}
\end{equation}

Substitute $\frac{\partial Loss}{\partial y_{j}}$ and $\frac{\partial Loss'}{\partial y_{j}}$ from Eq.~\ref{eq:dldw_{j}},

\begin{equation}
    x_{j} f_{j} (x_{j}, w_{j}) 
    =
    x'_{j} f_{j} (x'_{j}, w_{j}) 

\end{equation}

\zhijian{this part seems wrong....}

Since $f_j$ is a linear layer, $x_j f_j(x_j, w_j)$ is monotonous. When the equation holds, $ x_{j} $ must be equivalent as  $ x'_{j} $, which contradicts with the initial assumption $X \neq X, Y \neq Y'$.  

==> sections/notions.tex <==

\newcommand{\datax}[1]{\mathbb{#1}
